HyperGAN-CLIP: A Unified Framework for Domain Adaptation, Image Synthesis and Manipulation

Generative Adversarial Networks (GANs), particularly StyleGAN and its variants, have demonstrated remarkable capabilities in generating highly realistic images. Despite their success, adapting these models to diverse tasks such as domain adaptation, reference-guided synthesis, and text-guided manipulation with limited training data remains challenging. Towards this end, in this study, we present a novel framework that significantly extends the capabilities of a pre-trained StyleGAN by integrating CLIP space via hypernetworks. This integration allows dynamic adaptation of StyleGAN to new domains defined by reference images or textual descriptions. Additionally, we introduce a CLIP-guided discriminator that enhances the alignment between generated images and target domains, ensuring superior image quality. Our approach demonstrates unprecedented flexibility, enabling text-guided image manipulation without the need for text-specific training data and facilitating seamless style transfer. Comprehensive qualitative and quantitative evaluations confirm the robustness and superior performance of our framework compared to existing methods.

==> figures.tex <==
\begin{figure*}[!t]
  \centering
\includegraphics[width=0.97\linewidth]{figures/domain-adaptation-qual-new.pdf}
  \caption{\textbf{Comparison against the state-of-the-art few-shot domain adaptation methods}. Our proposed HyperGAN-CLIP model outperforms competing methods in accurately capturing the visual characteristics of the target domains. 
  }
  \label{fig:dom_ada_qual}
\end{figure*}

\begin{figure*}[!t]
    \centering
    \begin{subfigure}[t]{0.425\textwidth}
        \centering
        \begin{tabular}{ccc}
  $\;\;\quad$\small{Domain 1} & $\;\;\quad$\small{Domain 2} & $\;\;$\small{Hybrid}\\
  \multicolumn{3}{c}{\includegraphics[width=0.81\linewidth]{figures/mixing4.pdf}}
        \end{tabular}
        \caption{\textbf{Domain mixing.} Our approach can fuse multiple domains to create novel compositions. By averaging and re-scaling the CLIP embeddings of two target domains, we can generate images that blend characteristics from both.}
    \end{subfigure}%
    $\;\;$
    \begin{subfigure}[t]{0.555\textwidth}
        \centering
        \begin{tabular}{cccc}
  $\;\;\quad$\small{Adapted} & $\quad\qquad$\small{+Age} & $\quad\qquad$\small{+Smile} & $\quad$\small{+Pose}\\
  \multicolumn{4}{c}{\includegraphics[width=0.81\linewidth]{figures/Editing.drawio.pdf}}
  \end{tabular}
        \caption{\textbf{Semantic editing in target domains.} Since latent mapper is kept intact, our approach allows for using existing latent space discovery methods to perform semantic edits. We manipulate two sample face images from adapted domains by playing with age, smile, and pose using InterfaceGAN~\cite{shen2020interfacegan}.}
    \end{subfigure}
    \caption{\textbf{Capabilities of HyperGAN-CLIP in blending domains and performing semantic edits within adapted domains.}}
    \label{fig:capabilities}
\end{figure*}

\begin{figure*}[!t]
  \centering  \includegraphics[width=0.739\linewidth]{figures/image_based_editing_real.pdf}
  \caption{\textbf{Comparison with state-of-the-art reference-guided image synthesis approaches.} Our approach effectively transfers the style of the target image to the source image while effectively preserving identity compared to competing methods. %\basit{Should we update these figures with the results from residual features based method? Or we could also mention in a section where we talk about setting the interpolation coefficient between original and residual features. For these results, the coefficients could be 0. Refer approach 3.2 2nd last paragraph}
  }
  \label{fig:image_based_qualitative}
\end{figure*}

\begin{figure*}[!t]
  \centering
\includegraphics[width=\linewidth]{figures/text_based_editing.pdf}
\caption{\textbf{Comparisons with state-of-the-art text-guided image manipulation methods.} Our model shows remarkable versality in manipulating images across a diverse range of textual descriptions. The results vividly illustrate our model's ability to accurately apply changes based on target descriptions encompassing both single and multiple attributes. Compared to the competing approaches, our model preserves the identity of the input much better while successfully executing the desired manipulations. 
}
\label{fig:text_based_qualitative}
\end{figure*}
